A Simple and Scalable Representation for Graph Generation

Recently, there has been a surge of interest in employing neural networks for graph generation, a fundamental statistical learning problem with critical applications like molecule design and community analysis. However, most approaches encounter significant limitations when generating large-scale graphs. This is due to their requirement to output the full adjacency matrices whose size grows quadratically with the number of nodes. In response to this challenge, we introduce a new, simple, and scalable graph representation named gap encoded edge list (GEEL) that has a small representation size that aligns with the number of edges. In addition, GEEL significantly reduces the vocabulary size by incorporating the gap encoding and bandwidth restriction schemes. GEEL can be autoregressively generated with the incorporation of node positional encoding, and we further extend GEEL to deal with attributed graphs by designing a new grammar. Our findings reveal that the adoption of this compact representation not only enhances scalability but also bolsters performance by simplifying the graph generation process. We conduct a comprehensive evaluation across ten non-attributed and two molecular graph generation tasks, demonstrating the effectiveness of GEEL.

==> algorithm_attributed.tex <==
\begin{algorithm}[t]
\caption{Featured representation $L_F$ construction}
\label{algo:graph_featured}
\begin{algorithmic}[1]
\State \textbf{Input}: sorted list $L=((s_1, \tilde{t}_1), \dots, (s_M, \tilde{t}_M))$, ordered node list $v_i \in V^\pi$, ordered node feature matrix $x_i \in X^\pi$, ordered edge feature matrix $E$

\State Initialize an empty list $L_F$
\For{$i=1, \dots, N$}
    \State $L_F \gets L_F || x_i$ \Comment{Add node feature.}
        \State $(s_k, \tilde{t}_k) \gets L[0]$
        \If{$s_k \neq v_i$}
            \State $L_F \gets L_F || (1,0)$
            \State $s_{\operatorname{prev}} = 1$
        \Else
            \Do
                \State $\tilde{s}_k= \mathbbm{1}(s_k \neq s_{\operatorname{prev}})$ \Comment{Check whether the node is new or not.}
                \State $L_F \gets L_F || (\tilde{s}_k, \tilde{t}_k)$ \Comment{Add edge.}
                \State $L_F \gets L_F || E[s_k, s_k+\Tilde{t}_k] $ \Comment{Add edge feature ($t_k=s_k+\Tilde{t}_k)$).}
                \State $s_{\operatorname{prev}} = s_k$
                \State Pop $L[0]$
                \State $(s_k, \tilde{t}_k) \gets L[0]$
            \doWhile{$s_k \neq v_i$}
        % \Else
        %     \State $L_F \gets L_F || (1,0)$
        \EndIf
\EndFor


% \State $\pi(s_0)=0$
% \For{$(s_k, \Tilde{t}_k) \in L$}
%     \State $\operatorname{dist}= |\pi(s_k)-\pi(s_{k-1})|$
%     \If {$\operatorname{dist} = 0$} pass
%     \Else
%         \If {$\operatorname{dist} = 1$} \State $L_F \gets L_F || V^\pi[s_k]$ \Comment{Add node feature}
%         \Else
%             \State Initialize $i=\pi(s_{k-1})+1$
%             \While{$i \neq \pi(s_k)$}
%                 \State $L_F \gets L_F || V^\pi[i]$ \Comment{Add current node feature}
%                 \State $L_F \gets L_F || (1,0)$ \Comment{Add self-loop edge for masking}
%                 \State Set $i \gets i+1$
%             \EndWhile
%             \State $L_F \gets L_F || V^\pi[s_k]$ \Comment{Add node feature}
%         \EndIf
%     \EndIf
%     \State $L_F \gets L_F || (s_k, \Tilde{t}_k)$ \Comment{Add edge}
%     \State $L_F \gets E[s_k, s_k+\Tilde{t}_k]$ \Comment{Add edge feature where $e=(s_k, s_k+\Tilde{t}_k)$}
    
    

% \EndFor


\State \textbf{Output}: List with node and edge features $L_F$.
\end{algorithmic}
\end{algorithm}  

==> figure/fig_generated_graphs.tex <==
% \begin{figure}
% \centering
% \vspace{-.1in}
% \includegraphics[width=.9\linewidth, height=5cm]{example-image}
%     \caption{Generated samples.}\label{fig:gen_graphs}
%     \vspace{-.1in}
  
% \end{figure}

% \begin{figure}[t!]
%     \begin{subfigure}[t]{0.19\linewidth}
%     \centering
%       \includegraphics[width=\linewidth]{figure/generated_samples/GDSS_grid-train.png}
%       \subcaption{Train}
%       \label{subfig:com_train}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.19\linewidth}
%     \centering
%       \includegraphics[width=\linewidth]{figure/generated_samples/GDSS_grid-graphgen.png}
%       \subcaption{GraphGen \citep{goyal2020graphgen}}
%       \label{subfig:com_train}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.19\linewidth}
%     \centering
%       \includegraphics[width=\linewidth]{figure/generated_samples/GDSS_grid-gdss.png}
%       \subcaption{GDSS \citep{jo2022gdss}}
%       \label{subfig:com_train}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.19\linewidth}
%     \centering
%       \includegraphics[width=\linewidth]{figure/generated_samples/GDSS_grid-digress.png}
%       \subcaption{DiGress \citep{vignac2022digress}}
%       \label{subfig:com_train}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.19\linewidth}
%     \centering
%       \includegraphics[width=\linewidth]{figure/generated_samples/GDSS_grid-gcg.png}
%       \subcaption{\Algname (ours)}
%       \label{subfig:com_train}
%     \end{subfigure}
%     \caption{Generated samples for Community-small (top), and Grid (bottom) datasets.}
%   \label{fig:exp_main}
%   \vspace{-.1in}
% \end{figure}

==> figure/fig_intro_sparsity.tex <==
\begin{wrapfigure}{L}{0.5\textwidth}
\centering
\vspace{-.1in}
\includegraphics[width=.9\linewidth]{figure/fig_sparsity.pdf}
    \caption{\textbf{Edge list of a graph}. The edge list can represent graphs in a compact way by omitting zero elements. The shaded parts of the adjacency matrix denote zeros and the same colored part of the adjacency matrix and edge list signify the same edges.} \label{fig:intro_sparsity}
    \vspace{-.1in}
  
\end{wrapfigure}

==> figure/fig_main.tex <==
\begin{figure}[t]
\centering
\vspace{-.1in}
\includegraphics[width=\linewidth]{figure/overview.pdf}
    \caption{\textbf{Illustration of gap encoded edge list (GEEL)}. The same colored part of the graph and edge list signify the same edges. The representation size is $M$ and the vocabulary size is bounded by the square of bandwidth, $B^2$.} \label{fig: overview}
    % \sungs{Yellow lines should have arrows from bottom to up. How about showing the graph itself? The graph is disconnected, so weird.}}
    \vspace{-.1in}
  
\end{figure}

==> figure/fig_model.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
\centering
\vspace{-.1in}
\includegraphics[width=.9\linewidth]{example-image}
    \caption{Autoregressive generation of \Algname.} \label{fig:ab_sc_complexity}
    \vspace{-.1in}
  
\end{wrapfigure}

==> figure/fig_sca_complexity.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\centering
\vspace{-.1in}
\includegraphics[width=.9\linewidth]{figure/fig_sca_complexity.png}
    \caption{Inference time per graph.} \label{fig:ab_sc_complexity}
    \vspace{-.1in}
  
\end{wrapfigure}

==> figure/tab_ab_arch.tex <==
\begin{table}
\vspace{-.1in}
  \caption{\textbf{MMD results for different model architectures.}}\label{tab:ab_model}
  \centering
  \scalebox{0.8}{
    \begin{tabular}{lcccccccccccc}
    \toprule & \multicolumn{3}{c}{Planar} &\multicolumn{3}{c}{Lobster} & \multicolumn{3}{c}{Enzymes} & \multicolumn{3}{c}{Grid} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
    Backbone & Deg. & Clus. & Orb. & Deg. & Clus. & Orb. & Deg. & Clus. & Orb. & Deg. & Clus. & Orb.  \\
    \midrule
    LSTM & 0.001 & 0.004 & 0.001 & 0.007 & 0.002 & 0.005 & 0.008 & 0.015 & 0.006 & 0.000 & 0.000 & 0.000 \\
    Transformer & 0.003 & 0.004 & 0.001 & 0.004 & 0.000 & 0.003 & 0.005 & 0.015 & 0.005 & 0.000 & 0.000 & 0.000 \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> table/tab_ab_graphsize.tex <==
% \setlength\intextsep{0pt}
% \begin{wraptable}{R}{0.5\textwidth}
% \vspace{-.1in}
%   \caption{Average MMD on grid graphs with different average number of nodes.}
%   \label{tab:ab_quality_graph_size}

  % \centering
  %   \begin{tabular}{lccccc}
  %   \toprule
  %   Method & 0.5k & 1k & 5k & 10k  \\
  %   \midrule
  %   ER & 0.840 & 0.860 & 0.910 & 0.930 \\
  %   GRAN & 2.95$e^{-3}$ & 1.18$e^{-2}$  & 0.390 & 1.060 \\
  %   BiGG & 3.47$e^{-4}$ & 7.94$e^{-5}$ & \textbf{1.57$\boldsymbol{e^{-6}}$} & 6.39$e^{-6}$  \\
  %   \Algname & \textbf{3.38$\boldsymbol{e^{-4}}$} & \textbf{4.60$\boldsymbol{e^{-5}}$} & 2.00$e^{-6}$ & \textbf{0} \\
  %   \bottomrule
  % \end{tabular}

% \end{wraptable}

==> table/tab_ab_ordering.tex <==
% \begin{wraptable}{r}{0.45\textwidth}
% \vspace{-.1in}
%   \caption{Bandwidth and average MMD for different node orderings.}
%   \label{tab:ab_compression}
%   \centering
%   \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%     % \toprule & Ego-small & Community-small & Enzymes & Grid & Planar & SBM & Proteins \\
%     \toprule & \multicolumn{2}{c}{Enzymes} & \multicolumn{2}{c}{Ego} & \multicolumn{2}{c}{Grid} \\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%     & \multicolumn{2}{c}{$|V|_{\operatorname{max}}=125$} & \multicolumn{2}{c}{$|V|_{\operatorname{max}}=399$} & \multicolumn{2}{c}{$|V|_{\operatorname{max}}=400$} \\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%     Method & BW & MMD & BW & MMD & BW & MMD  \\
%     \midrule
%     DFS & 124 & 0.013 & 398 & & 360 &\\
%     Random & 112 & 0.011 & 396& & 347 &\\
%     BFS  & 21 & 0.010 & 266 & & 33 &\\
%     C-M & 19 & 0.010 & 241 & & 19 &\\
%     \bottomrule
%   \end{tabular}
%   }
% \end{wraptable}

==> table/tab_ab_rep.tex <==
% \begin{wraptable}{l}{0.45\textwidth}
% \vspace{-.1in}
%   \caption{Vocab size and sequence length for different representations.}
%   \label{tab:ab_representation}
%   \centering
%   \scalebox{0.8}{
%     \begin{tabular}{cccc}
%     \toprule
%     Representation & Sequence length & Vocab size  \\
%     \midrule
%     Flattened adj. matrix & $N^2$  & $2$ \\
%     Edge list & $M$ & $N*B$  \\
%     Double relative edge list & $N+M$ & $B*B$ \\
%     \Algname (Ours) & $N+M$ & $2*B$ \\
%     \bottomrule
%   \end{tabular}
%   }
% \end{wraptable}
\begin{table}
% \vspace{-.1in}
  \caption{\textbf{Average MMD for different representations}. We adopted LSTM as a model architecture and OOM denotes out-of-memory error.}
  \label{tab:ab_representation}
  \centering
  \scalebox{0.8}{
    \begin{tabular}{lcccccc}
    \toprule
    % \multicolumn{3}{c}{Representation} & \multicolumn{2}{c}{Complexity} & \multicolumn{3}{c}{Avg. MMD} \\
    Representation & Sequence length & Vocab size & Community-small & Grid & Point  \\
    \midrule
    Flattened adj. matrix & $N^2$ & $2$ & 0.029 & OOM & OOM  \\
    Edge list &  $M$ & $N^2$ & 0.010 & 0.000 & OOM \\
    Edge list + intra-edge gap &  $M$ &$NB$ & 0.013  & 0.000 & OOM \\
    \midrule
    \Repname &  $M$ & $B^2$ & 0.016 & 0.000  & 0.044 \\
    \bottomrule
  \end{tabular}
  }
\end{table}


==> table/tab_ab_sparsity.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\vspace{-.1in}
  \caption{\textbf{Average MMD with decreasing sparsity}.} \label{tab:ab_sparsity}
  \centering
  \scalebox{0.8}{
    \begin{tabular}{cccccccc}
    \toprule
     & 1\% & 2\% & 5\% & 10\% & 20\% & 50\%  \\
    \midrule
    GRAN &  &  &&&&\\
    BiGG & &  &&&& \\
    \Algname (Ours) &  & &&&& \\
    \bottomrule
  \end{tabular}
  }
\end{wraptable}

==> table/tab_sca_runtime.tex <==

  \centering
    \begin{tabular}{llccc}
    \toprule
    Method & Type & Enzymes & Planar & Grid \\
    \midrule
    GRAN  & Auto. Reg. & \phantom{0}0.24 & \phantom{0}0.66 & \phantom{0}1.39   \\
    BiGG & Auto. Reg. & \phantom{0}2.70 & \phantom{0}0.61 & \phantom{0}3.58  \\
    GDSS & Diffusion & 15.21 & 15.25  & 30.89  \\
    DiGress & Diffusion & \phantom{0}8.82 & 12.09 & 32.29  \\
    %\midrule
    \Algname (ours) & Auto. Reg. & \phantom{0}\textbf{0.12} & \phantom{0}\textbf{0.25} & \phantom{0}\textbf{1.11}  \\
    \bottomrule
  \end{tabular}

